A Polynomial-time Solution for Robust Registration with Extreme Outlier Rates

We propose a robust approach for the registration of two sets of 3D points in the presence of a large amount of outliers. Our first contribution is to reformulate the registration problem using a Truncated Least Squares (TLS) cost that makes the estimation insensitive to a large fraction of spurious point-to-point correspondences. The second contribution is a general framework to decouple rotation, translation, and scale estimation, which allows solving in cascade for the three transformations. Since each subproblem (scale, rotation, and translation estimation) is still non-convex and combinatorial in nature, out third contribution is to show that (i) TLS scale and (component-wise) translation estimation can be solved exactly and in polynomial time via an adaptive voting scheme, (ii) TLS rotation estimation can be relaxed to a semidefinite program and the relaxation is tight in practice, even in the presence of an extreme amount of outliers. We validate the proposed algorithm, named TEASER (Truncated least squares Estimation And SEmidefinite Relaxation), in standard registration benchmarks showing that the algorithm outperforms RANSAC and robust local optimization techniques, and favorably compares with Branch-and-Bound methods, while being a polynomial-time algorithm. TEASER can tolerate up to 99% outliers and returns highly-accurate solutions.

==> fig-benchmarkUnknownScale.tex <==
%!TEX root = main.tex

\begin{figure}[h]
	\begin{center}
	\begin{minipage}{\textwidth}
	\hspace{-0.2cm}
	\begin{tabular}{ccc}%
		\myhspace
			\begin{minipage}{3cm}%
			\centering%
			\includegraphics[width=\columnwidth]{scale_err_unknown_scale_ss.pdf} \\
			(a) Scale error
			\end{minipage}
		& 
		\myhspace
			\begin{minipage}{3cm}%
			\centering%
			\includegraphics[width=\columnwidth]{rot_err_unknown_scale_ss.pdf} \\
			(b) Rotation error
			\end{minipage}
			& 
			\myhspace
			\begin{minipage}{3cm}%
			\centering%
			\includegraphics[width=\columnwidth]{trans_err_unknown_scale_ss.pdf} \\
			(c) Translation error
			\end{minipage}
		\end{tabular}
	\end{minipage}
	\begin{minipage}{\textwidth}
	\end{minipage}
	\vspace{-3mm} 
	\caption{Benchmark results for registration with unknown scale.
	 \label{fig:benchmarkUnknownScale}}
	\vspace{-8mm} 
	\end{center}
\end{figure}

==> guarantees.tex <==
%!TEX root = main.tex

\section{Performance Guarantees}
\label{sec:guarantees}

\grayout{
\begin{theorem}[Efficiency of Scale Estimation]
Scale estimation does not reject inliers.
\end{theorem}

\begin{theorem}[Efficiency of Rotation Estimation]
Rotation estimation does not reject inliers.
\end{theorem}

Approximate: is that an upper or lower bound?

\vspace{1cm}
}

==> scaleEstimation_old.tex <==
%!TEX root = main.tex

\subsection{Robust Scale Estimation}
\label{sec:scaleEstimation}

In this section we use the rotation and translation invariant measurements in eq.~\eqref{eq:TRIM} to 
estimate the scale $s$. The generative model~\eqref{eq:TRIM} describes measurements $s_{ij}$ affected 
by bounded noise $|\eps^s_{ij}| \leq \alpha_{ij}$ including potential outliers (when $o^s_{ij} \neq 0$).
Again, we estimate the scale given the measurements $s_{ij}$ and the bounds $\alpha_{ij}$ using a 
\TLS estimator:
\bea
\label{eq:TLSscale}
\hats = \argmin_{s} \sumAllIM \min\left( \frac{  (  s-s_k )^2 }{  \alpha^2_k }  \;,\; \barcsq \right)
\eea
where for simplicity we numbered the measurements from $1$ to $K = |\calE|$ and adopted the notation $s_k$ instead of $s_{ij}$.
% From the previous section we have a bunch of measurements of the scale, potentially affected by outliers:
% \bea
% s_k \doteq \frac{  \|  \vb_{ij} \| }{  \|  \va_{ij} \| }  = s + \hat{o}_{ij} 
% \eea
% \TLS estimator:
% %
% \bea
% \label{eq:TLSscale}
% % s^\star = \argmin_{s} \sumAllPoints \min\left( (s - s_k)^2 , \barcsq \right)
% s^\star = \argmin_{s,\theta_k \in \{-1,+1\}} 
% \sumAllPoints \frac{(1+\theta_k)}{2}  \frac{(s - s_k)^2}{\sigma_s^2}  + \frac{(1-\theta_k)}{2}  \barcsq 
% \eea

The following theorem relates the \TLS estimator~\eqref{eq:TLSscale} to \emph{consensus maximization}, 
a popular framework for robust estimation in vision~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}. 
This is instrumental to design a polynomial-time solution for~\eqref{eq:TLSscale} (\prettyref{thm:maxConsensusAlgo}). 

\begin{theorem}[\TLS Scale Estimation]\label{thm:scalarTLS}
Whenever the consensus set is unique, the optimal solution $\hats$ of the \TLS scale estimation~\eqref{eq:TLSscale} can be computed in two steps:
\begin{enumerate}
\item Consensus maximization: %Find the maximum consensus set: 
\beq
\label{eq:consensusMax}
(z^\star, \calS^\star) = \argmax_z \sumAllPoints \calI\left( \frac{(z - s_k)}{\alpha_k^2} \leq \barcsq \right)
\eeq
where $\calI$ is the indicator function, which is $1$ when the argument is true and zero otherwise.
Problem~\eqref{eq:consensusMax} returns a (typically non unique) $z^\star$ and a consensus set $\calS^\star$ 
that are such that $\frac{(z^\star - s_k)}{\alpha_k^2} \leq \barcsq$ for all $k\in \calS^\star$.
\item Least squares scale estimation over the consensus set: 
\beq
\hats = \left(\sum_{k\in \calS^\star } \frac{1}{\alpha_k^2}\right)\inv  \sum_{k\in \calS^\star} \frac{1}{\alpha_k^2} s_k
\eeq
\end{enumerate}
\end{theorem}
% consensus maximization is a popular framework~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}, 
A proof of~\prettyref{thm:scalarTLS} is  given in Appendix~\ref{sec:proof:scalarTLS}.

While~\prettyref{thm:scalarTLS} draws an interesting connection between two robust estimation frameworks, 
it appear not to provide a tractable algorithmic solution, since exact consensus maximization~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration} is intractable in general. 
Our insight here is that, while consensus maximization is hard in general, it can be solved in polynomial time in the 
scalar case. 

An intuition is given in Fig.~\ref{fig:consensusMax},  
% ========================
\input{fig-consensusMax} 
% ========================

Problem~\eqref{eq:consensusMax} can be solved exactly using the adaptive voting scheme described in Algorithm~\ref{alg:adaptiveVoting}.

\begin{algorithm}[h]
\SetAlgoLined
\textbf{Input:} \ $s_k, \beta_k$\; 
\textbf{Output:} \  $(\calS^\star,y^\star)$, where the maximum consensus set $\calS^\star$  and $y^\star$ solve the consensus maximization~\eqref{eq:consensusMax}\;
\% Define vector and sort \\
\indent $\vv = [s_1 - \beta_1, s_1 + \beta_1,\ldots,s_\nrPoints - \beta_\nrPoints, s_\nrPoints + \beta_\nrPoints]$ \\
\indent $\vv = \text{sort}(\vv)$ \\
\% Compute middle points \\%\;
\For{$i = 1,\ldots,2\nrPoints-1$}{$m_i = \frac{\vv_{2i-1} + \vv_{2i}}{2}$}
 \% Voting \\%\;
 \For{$i = 1,\ldots,2\nrPoints-1$}{
 	$\calS_i = \emptyset$\\
 	\For{$k = 1,\ldots,\nrPoints$}{
		\If{$m_i \in [s_k - \beta_k, s_k + \beta_k]$}{
			$\calS_i = \calS_i \cup \{k\}$ \% add to consensus set\\
		}
	}
}
\% Pick largest consensus set\\
$i^\star = \argmax_i |\calS_i|$\\
 \textbf{return:} $(\calS_i, m_i)$ 
 % \While{g(S) > R}{
 %  $S_{i+1} \leftarrow S_i \cup \{ \underset{a \in G \backslash S_i}{\text{arg min}} \ {\rm{MG}}_g(a | S_i)  \}$ \;
 % }
 \caption{Adaptive Voting.\label{alg:adaptiveVoting}}
\end{algorithm} 


\begin{theorem}[Optimality of Algorithm~\ref{alg:adaptiveVoting}]\label{thm:maxConsensusAlgo}
Algorithm~\ref{alg:adaptiveVoting} computes an optimal solution for Problem~\eqref{eq:consensusMax} 
in $\calO(K^2)$.
\end{theorem}

Proof is given in Appendix~\ref{sec:proof:maxConsensusAlgo}.


estimate must be positive: convex combination of positive quantities
